A Survey of Data Augmentation Approaches for NLP

Data augmentation has recently seen increased interest in NLP due to more work in low-resource domains, new tasks, and the popularity of large-scale neural networks that require large amounts of training data. Despite this recent upsurge, this area is still relatively underexplored, perhaps due to the challenges posed by the discrete nature of language data. In this paper, we present a comprehensive and unifying survey of data augmentation for NLP by summarizing the literature in a structured manner. We first introduce and motivate data augmentation for NLP, and then discuss major methodologically representative approaches. Next, we highlight techniques that are used for popular NLP applications and tasks. We conclude by outlining current challenges and directions for future research. Overall, our paper aims to clarify the landscape of existing literature in data augmentation for NLP and motivate additional work in this area. We also present a GitHub repository with a paper list that will be continuously updated at https://github.com/styfeng/DataAug4NLP

==> sections/abstract_tutorial.tex <==
%\section*{Abstract}
% Topic and Content
%\steven{the short-form of the whole tutorial (DAApprNLP) sounds quite convoluted and does not roll off the tongue LOL - I propose something simple like DA4NLP} %SGTM - jason idk who wrote daapprnlp
Data augmentation (\textsc{DA}) has received active attention in recent machine learning research in the form of well-received, general-purpose techniques such as MixUp \cite{zhang2018mixup} and UDA \cite{xie2019unsupervised}. 
These techniques, however, are often first explored in computer vision, and the adaptation of data augmentation for natural language processing (NLP) seems secondary and comparatively under-explored, perhaps due to challenges presented by the discrete nature of language data.
% However, many of these are often first experimented with on continuous input including vision benchmarks and classification such as CIFAR-100, with their adaptation to natural
% language inputs and NL-specific task families being slow-moving and
% under-explored. This is due to a combination of lack of attention\footnote{We mean the layman sense of the word.} and the difficulties involved with language.
% Despite these challenges, data augmentation has recently been gained more attention in NLP, showing potential to improve model performance \cite{kobayashi-2018-contextual} and robustness \cite{, and

Despite the challenges in devising \textsc{DA} methods in NLP, there has been both increased interest and demand for \textsc{DA}. As the field of NLP continues to grow due to the off-the-shelf availability of large pre-trained models, there are increasingly more tasks and domains that researchers aim to explore. Many of these domains are low-resource, and therefore have a paucity of training examples, creating many use-cases for which \textsc{DA} could play an important role. 
Particularly, for many non-classification tasks in NLP (e.g., span-based tasks and generation), \textsc{DA} research is relatively sparse at the moment despite their ubiquity in real-world settings such as conversational AI.

%There is increasing potential for \textsc{DA} due to more work in low-resource domains which may not have sufficient data available to begin with. At least a few in-domain examples are required for many NLP tasks, as the involved models must learn domain-specific properties to be effective and achieve the desired results.

% NLP has a wide range of non-classification tasks such as span-based tasks and generation. These would ideally bear the potential to both present new challenges and motivate new research directions w.r.t. augmentation. %However, one finds limited forays on these lines. For example, there has been limited work on augmentation for generation tasks. 

Our tutorial aims to sensitize the NLP community towards this growing area of work by giving an introductory overview of \textsc{DA} techniques and the motivation behind developing them for NLP. First, we will present what DA is and discuss its motivation and challenges for NLP.
Next, we will describe common task-agnostic DA techniques and their strengths and drawbacks.
Finally, we will introduce specialized applications of DA and conclude with future directions (e.g. facilitate self-supervised learning techniques).
We hope to draw further attention, elicit broader interest, and motivate additional work in \textsc{DA}, particularly for NLP.
% To provide a complete discussion of the general \textsc{DA} methods, we will first introduce several popular methods for the computer vision benchmarks~\citep{}, which bring significant improvements for model performance~\cite{} and model robustness under distribution shift~\cite{}. Next, we will introduce the specific challenges in language processing that \textsc{DA} can address, such as improving model performance for low-resource languages~\cite{} and adapting models to different domains~\cite{}.

==> sections/backup_techniquesandmethods.tex <==
%\vspace{1.5mm} \noindent \textbf{Rule-based techniques.} \label{rulebased}
%We now discuss some major task-agnostic data augmentation techniques.
We now discuss some methodologically representative DA techniques which are relevant to all tasks via the extensibility of their formulation.\footnote{\label{note1}Table \ref{table:comparison} in Appendix \ref{sec:appendix_table_typology} compares several \textsc{DA} methods by various aspects relating to their applicability and requirements.}

\subsection{Rule-Based Techniques}\label{subsec:rule-based}
\textit{Feature space DA} (FSDA) approaches create augmented examples in the feature space of the model rather than input data. Many few-shot learning approaches \cite{hariharan2017low,schwartz2018delta} estimate "analogy" transformations in feature space between examples from known classes and leverage these to augment examples for novel classes. \citet{paschali2019data} use iterative affine transformations and projections to maximally "stretch" an example along the class-manifold.

\citet{wei-zou-2019-eda} propose \textsc{Easy Data Augmentation (EDA)}, which is a set of simple token-level random perturbation operations for DA: \textit{synonym replacement} \cite{10.5555/2969239.2969312}, \textit{random insertion}, \textit{random deletion}, and \textit{random swap}. They show improved performance using these simple DA techniques for various text classification tasks.

For paraphrase identification, which is a sentence pair classification task, \citet{chen-etal-2020-finding} construct a signed graph over the entire training set, with individual sentences as nodes and pair labels as signed edges. They use intuitions from structural balance theory along with transitivity to synthesize augmented sentence pair examples from this graph.

Motivated by image cropping and rotation used for \textsc{DA} in vision, \citet{csahin2019data} propose \emph{dependency tree morphing}. For dependency-annotated sentences, children of the same parent are mutually swapped (à la rotation) or some deleted (à la cropping), as seen in Figure \ref{img-deptreemorph}.

\begin{figure}
\centering
\begin{tabular}{@{}ll@{}}
\includegraphics[width=0.40\textwidth]{Images/SahinSteedman.png}\\
\end{tabular}
\vspace{-0.8\abovedisplayskip}
  \caption{\label{img-deptreemorph} \emph{Dependency tree morphing} \textsc{DA} applied to a Turkish sentence, \citet{csahin2019data}}
\vspace{-2ex}
\end{figure} 


\subsection{Example Interpolation Techniques}\label{subsec:example_interpolation}
Another class of \textsc{DA} techniques, pioneered by \textsc{MixUp} \cite{zhang2018mixup}, interpolates the inputs and labels of two or more real examples, a paradigm with theoretical underpinnings \cite{chapelle2001vicinal}. This class of techniques is also sometimes referred to as \emph{Mixed Sample Data Augmentation} (MSDA). Ensuing work has explored interpolating inner components \cite{verma2019manifold,faramarzi2020patchup}, more general mixing schemes \cite{guo2020nonlinear} and adding adversaries \cite{beckham2019adversarial}. Another class of extensions of \textsc{MixUp} which has been growing in the vision community attempt to fuse raw input image pairs together into a single input image, rather than improve the continuous interpolation mechanism. Examples of this paradigm include \textsc{CutMix} \cite{yun2019cutmix}, \textsc{CutOut} \cite{devries2017improved} and \textsc{Copy-Paste} \cite{ghiasi2020simple}. For instance, \textsc{CutMix} replaces a small sub-region of Image A with a patch sampled from Image B, with the labels mixed in proportion to sub-region sizes.

A bottleneck to using \textsc{MixUp} for NLP tasks was the requirement of continuous inputs. This has been overcome by padding and mixing embeddings or higher hidden layers \cite{chen2020mixtext}. Later variants propose speech-tailored mixing schemes \cite{jindalspeechmix} and interpolation with adversarial examples \cite{cheng-etal-2020-advaug}, among others.

\textsc{Seq2MixUp} \cite{guo-etal-2020-sequence} generalizes \textsc{MixUp} for sequence transduction tasks in two ways - the "hard" version samples a binary mask (from a Bernoulli with a $\beta(\alpha,\alpha)$ prior) and picks from one of two sequences at each token position, while the "soft" version softly interpolates between sequences based on a coefficient sampled from $\beta(\alpha,\alpha)$. The "soft" version is found to outperform the "hard" version and earlier interpolation-based techniques like \textsc{SwitchOut} \cite{wang-etal-2018-switchout}.

\begin{figure}%[!ht]
\centering
\begin{tabular}{@{}ll@{}}
\includegraphics[width=0.36\textwidth]{Images/ContextualKobayashi.png}\\
\end{tabular}
\vspace{-0.8\abovedisplayskip}
  \caption{\label{tab:qualitative_1} \emph{Contextual Augmentation}, \citet{kobayashi-2018-contextual}}
\vspace{-2ex}
\end{figure} 

\subsection{Model-Based Techniques}\label{subsec:model_based}
Seq2seq and language models have also been used for \textsc{DA}. The popular \textsc{backtranslation} method \cite{sennrich-etal-2016-improving} translates a sequence into another language and then back into the original language. Pretrained language models such as RNNs \cite{kobayashi-2018-contextual} and transformers \cite{yang2020g} have also been used to create augmented examples by reconstructing sub-parts of real data.

\citet{kobayashi-2018-contextual} generate augmented examples by replacing words with others randomly drawn according to the recurrent language model's distribution based on the current context (illustration in Figure \ref{tab:qualitative_1}). \citet{gao-etal-2019-soft} advocate retaining the full distribution through "soft" augmented examples, showing gains on machine translation.

\citet{nie-etal-2020-named} augment word representations with a context-sensitive attention based mixture of their semantic neighbors from a pre-trained embedding space. They show this approach is effective for NER on social media text.

Inspired by denoising autoencoders, \citet{ng-etal-2020-ssmba} use a corrupt-and-reconstruct approach, with the corruption function $q(x'|x)$ masking an arbitrary number of word positions and the reconstruction function $r(x|x')$ unmasking them using BERT \cite{devlin2019bert}. Their approach works well on domain-shifted test sets across 9 datasets and 3 tasks (sentiment analysis, NLI, and NMT).% (They do not evaluate on the IID case, since their goal is to improve OOD generalization)

\citet{feng-etal-2019-keep} propose a method called \textsc{Semantic Text Exchange} (STE) which adjusts the overall semantics of a piece of text to fit the context of a new word or phrase that is inserted called the \textit{replacement entity (RE)}. They do so by using a system called SMERTI and a masked language model approach (Figure \ref{fig:SMERTI}). While not proposed directly as a DA method, it can be used for such purposes, as investigated in \citet{feng2020genaug}.

Rather than starting from an existing example and modifying it, some model-based \textsc{DA} approaches directly estimate a generative process from the training set and sample from it. \citet{anaby2020not} learn a label-conditioned generator by finetuning GPT-2 \cite{radford2019language} on the training data, using this to generate candidate examples per class. A classifier trained on the original training set is then used to select top $k$ candidate examples which confidently belong to the respective class for augmentation. \citet{quteineh2020textual} use a similar label-conditioned GPT-2 generation method, and demonstrate its effectiveness as a \textsc{DA} method in an active learning setup.

Other approaches include syntactic paraphrasing models \cite{iyyer2018adversarial}, augmenting misclassified examples \cite{dreossi2018counterexample} and guided generation using large-scale generative language models \cite{liu2020databoost,liu2020offensive}. Models can also learn to combine together simpler DA primitives \cite{cubuk2018autoaugment,ratner2017learning} or add humans-in-the-loop (HITL) \cite{kaushik2020learning,kaushik2021explaining}.

%\subsection{Historical}
%\steven{Really think we should just remove this historical section. I think we were going to talk about older DA techniques here but our survey is on "modern approaches" and this would be a waste of space.}\varun{Sure, I think we can remove it.}

\begin{figure}
\begin{tabular}{@{}ll@{}}
\includegraphics[width=0.48\textwidth]{Images/overall_architecture.png}
\end{tabular}
  \caption{\label{fig:SMERTI} SMERTI pipeline for STE, where \emph{S} is modified to fit the semantic context of \emph{RE}, \citet{feng-etal-2019-keep}}
\end{figure}


\begin{comment}
\begin{table*}[t!]
\caption{Timeline of something. \steven{Note: this needs to be modified for DA and completed. It is also too large (font is huge) and can probably be shrunk to save space. Can also remove this in the end if unnecessary/incoherent.}}
\centering
\begin{minipage}[t]{\linewidth}
\color{gray}
\rule{\linewidth}{1pt}
\ytl{1947}{AT and T Bell Labs develop the idea of cellular phones}
\ytl{1968}{First appearance of the term \emph{`data augmentation'} in print.}
\ytl{1971}{Busicom 'Handy-LE' Calculator}
\ytl{2001}{VRM proposed \cite{chapelle2001vicinal}}
\ytl{1978}{Parker Bros. Merlin Computer Toy}
\ytl{1981}{Osborne 1 Portable Computer}
\ytl{1982}{Grid Compass 1100 Clamshell Laptop}
\ytl{2019}{EDA \cite{wei-zou-2019-eda}, UDA \cite{xie2019unsupervised} repos both cross 500+ stars}
\ytl{1984}{Psion Organiser Handheld Computer}
\ytl{1991}{Psion Series 3 Minicomputer}
\bigskip
\rule{\linewidth}{1pt}%
\end{minipage}%
\end{table*}
\end{comment}

==> sections/description_tutorial.tex <==
%\url{https://www.aclweb.org/anthology/2020.acl-tutorials.7.pdf}
%We can use this as one of the guides for writing this and other sections.

\subsection{Introduction to Data Augmentation}
\noindent \textbf{What is data augmentation?} \label{rulebased}
Data augmentation (\textsc{DA}) refers to strategies for increasing the diversity of training examples without explicitly collecting new data. 
Most strategies either add slightly modified copies of already existing data or create synthetic data from existing data, aiming for augmented data to act as a regularizer and reducing overfitting when training machine learning models \cite{shorten2019survey}. %\varun{IMHO we shouldn't be saying these kind of things without giving a proper citation. Regularization can mean a lot of things and its not immediately obvious which one DA is equivalent to. Overfitting is also a pretty broad term tbh - esp with already overcapacity deep models the whole train-test typical error curve doesnt hold and things are pretty different - sometimes they are even bimodal.} 

Data augmentation has been commonly used in computer vision, where techniques such as cropping, flipping, and color jittering are a standard component of model training.
However, in NLP, where the input space is discrete rather than continuous, how to generate new examples without changing their original meaning is not as obvious. 

\vspace{1.5mm} \noindent \textbf{What are the goals and trade-offs?} \label{rulebased}
Despite the challenges of manipulating text, many DA techniques for NLP have been proposed, ranging from simple rule-based manipulations \cite{10.5555/2969239.2969312} to more complicated generative approaches \cite{liu2020databoost}.
As DA aims to provide an alternative to collecting more data, an ideal DA technique should be both easy-to-implement and improve model performance on the desired task.
Most DA techniques offer some trade-offs between these two objectives.
Rule-based techniques are easy-to-implement but usually offer only incremental performance improvements 
\cite{li-etal-2017-robust,wei-zou-2019-eda}. 
Techniques that leverage trained models (e.g. back-translation \cite{sennrich-etal-2016-improving}) may be more costly to implement but potentially introduce more variation in the training data, leading to better performance boosts.
Finally, model-based techniques customized for downstream tasks can have the strongest desired effects on performance but be the most difficult to develop and execute.
% To mimic the widespreadness of DA in computer vision, techniques should be easy-to-implement, meaning-preserving, and improve model performance on downstream tasks.
% Choosing the correct data augmentation technique to use often involves considering some trade-offs between these three factors.
% For instance, rule-based techniques are often the easiest to implement but introduce noisy training data only improve model performance marginally.
% Model-based techniques can introduce greater variation in the training set but can be costly to implement.
% And often, techniques hand-crafted for downstream tasks offer the greatest performance improvements but can both require creativity to develop and be complex to implement. 
 
%DA is important for NLP as the development of models has led to increased work in low-resource domains with little data. Models must be finetuned to these to pick up domain-specific characteristics. For example, for text generation, it must pick up aspects related to length, style (e.g. formality and sentiment), and vocabulary, to generate text that imitates the language of the domain.
%\steven{actually screw this paragraph, i realized we summarize this in the intro}

% DA has seen less work in NLP with generally limited techniques compared to computer vision (CV). One explanation is that the discrete nature of NLP makes it difficult to adjust the data and produce meaningful augmented examples. Unlike CV, where simple techniques such as croppings, color adjustment, and geometric transformations are prevalent for many tasks, techniques for NLP must typically be more careful and involved. For example, for text generation, the augmented examples should likely maintain grammaticality, fluency, and coherence to be effective.
% \steven{added the couple paragraphs above based on some quick thoughts, feel free to modify or scrap whatever}

% \jason{One concern that I have right now is that it feels like we are too much just surveying the field instead of actually teaching someone about \textsc{DA}. Maybe we should have a section on like what makes a data augmentation technique good (IG this could go in 2.1). Or we could have some easy to run code examples (e.g., \url{https://github.com/QData/TextAttack})}
% \varun{I think this concern makes a lot of sense.}
% \varun{Maybe just like our reading list, we could also have a list of Good Repos/Implementations which actually someone can get working and use e.g the above one}

% \steven{we really need to finish the subsections below (2.1.1-2.1.3) or scrap them}
% \subsubsection{What makes a \textsc{DA} method ``good"?}

% \subsubsection{How to use augmented examples?}
% \citet{hoffer2020augment} show that using actual examples with their augmented variants to create larger minibatches leads to a better training schedule \varun{need to makes this sound better.}\steven{is this section necessary? what exactly will be discussed here?}

% \subsubsection{Why does \textsc{DA} work?}
% \varun{Equivalence to Regularization is one view}
% \citet{xie2017data} establish a link between augmentation and smoothing for n-gram language models.\steven{similar to above, but is this section necessary? what exactly will be discussed here?} \varun{IMHO Yes... We cannot just talk about DA and a bunch of methods, and also claim things about DA being regularization and DA helping training etc without referring to work which in some way justifies these claims and also proves specifically why. This section was also motivated by Jason's earlier commment. What should be discussed here is - why does DA work based on ML/Stats/Learning Theory intuitions/claims and proofs - and what existing variance reduction techniques (e.g regularization) it can be reduced to.}

\subsection{What are Common \textsc{DA} Techniques and Their Applications?}
% Whereas data augmentation is more straightforward in vision since the input space is continuous (e.g., rotation, flipping, color jittering), text data is discrete and so it is unclear how to generate similar training examples while maintaining the original meaning of the sentence.
%Parallel Data Augmentation for Formality Style Transfer Yi Zhang, Tao Ge and Xu SUN
Although the goal of \textsc{DA} is to artificially increase the training set in order to facilitate learning a specific task, many common \textsc{DA} techniques are \textit{task-agnostic} in that they generally aim to create new examples with similar meaning to original training data and could be potentially used in a variety of downstream tasks. 
This section summarizes common task-agnostic \textsc{DA} techniques in NLP.

\vspace{1.5mm} \noindent \textbf{Rule-based techniques.} \label{rulebased}
Perhaps the simplest class of \textsc{DA} techniques is rule-based token manipulation. Common methods include: \textbf{(1) Word Dropout} \cite{sennrich-etal-2016-edinburgh} randomly drops words with probability $p$, \textbf{(2) Token Substitution} \cite{wang-yang-2015-thats,10.5555/2969239.2969312} replaces words with their synonyms (which can use a knowledge-base \cite{miller1995wordnet,pavlick-etal-2015-ppdb}), and \textbf{(3) Token Shuffling} swaps the position of tokens in a sequence \cite{wei-zou-2019-eda}. Other techniques include linguistically-motivated noise \cite{li-etal-2017-robust}, syntactic transformations \cite{min-etal-2020-syntactic}, and replacing sentence fragments based on linguistic patterns \cite{andreas-2020-good}.
%other fragments that appear in similar environments

\vspace{1.5mm} \noindent \textbf{Example interpolation techniques.}
Another class of \textsc{DA} techniques, pioneered by MixUp \cite{zhang2018mixup}, interpolates the inputs and labels of two or more real examples, a paradigm wih theoretical underpinnings \cite{chapelle2001vicinal}.
Following work has explored interpolating inner components \cite{verma2019manifold,faramarzi2020patchup}, more general mixing schemes \cite{guo2020nonlinear}, adding adversaries \cite{beckham2019adversarial}, and speech-based mixing schemes \cite{jindalspeechmix}.
% A bottleneck to using MixUp for NLP tasks right-away was the requirement of continuous inputs - this has been eventually overcome by padding and mixing embeddings or higher hidden layers \cite{chen2020mixtext}. Later variants propose speech-tailored mixing schemes \cite{jindalspeechmix}, interpolation with adversarial examples \cite{cheng2020advaug} inter alia.

%Interpolating Examples - Mixup and its variants
%\cite{zhang2018mixup,verma2019manifold,jindalspeechmix,chen2020mixtext}

\vspace{1.5mm} \noindent \textbf{Model-based techniques.}
Sequence-to-sequence and language models have also been used for \textsc{DA}.
The popular \textit{backtranslation} technique \cite{sennrich-etal-2016-improving} translates a sequence into another language and then back into the original language. 
Pre-trained language models such as RNNs \cite{kobayashi-2018-contextual} and transformers \cite{yang2020g} have also been used to create augmented examples by reconstructing sub-parts of real data.
Other approaches include syntatic paraphrasing models \cite{iyyer2018adversarial}, augmenting misclassified examples \cite{dreossi2018counterexample} and guided generation using large-scale generative language models \cite{liu2020databoost,liu2020offensive}. Models can also learn to combine together simpler DA primitives \cite{cubuk2018autoaugment,ratner2017learning}.
% Models capable of fluently performing conditional generation or reconstruction, e.g large pre-trained LMs such as GPT-2, have also been used to construct augmented examples \cite{yang2020g} - typically through reconstruction from sub-parts of the input.
%contextual augmentation

% \jason{Given space constraints, I think everything below here in section 2.2 could be shortened to two sentences. } \steven{I agree. I think 2.2 overall is too long and seems to be mainly just a listing of numerous papers and techniques (which isn't necessarily bad per se). I am less familiar with the content here so I will leave it up to you guys to cut. Also does anybody know if the references are included in the 6 page total limit? It would make a huge deal because we have over 2 pages of references already}
% Paraphrasing based on syntax provide another route to generate augmented examples. In \citet{iyyer2018adversarial},  a unsupervised model is learnt to generate paraphrases satisfying a target constituency-subtree as template. Alternative methods in ensuing work include exemplars \cite{chen2019controllable},  pre-ordering \cite{goyal2020neural}, dependency tree morphing \cite{csahin2019data} and Latent Variable PCFGs\footnote{Probabilistic Context-Free Grammars} \cite{narayan2016paraphrase}.

% %\varun{Comment for self: Fix the subsubsections and make them into just single sentences by linearizing them.}
% %\vspace{1.5mm} \noindent \textbf{}

% \jason{If these are all vision, they should perhaps not be included here.} \varun{Its true exps might be in large part vision [some may have nlp exps too gotta read carefully] but formulations are pretty generic and domain-agnostic as long as some set of primitives is defined.}
% Models can also  learn how to combine simpler \textsc{DA} primitives into a composite \textsc{DA} method or ``policy" for each example. This is exemplified in approaches like Transformation Functions \cite{ratner2017learning}, AutoAugment \cite{cubuk2018autoaugment}, PBA \cite{ho2019population} and RandAugment \cite{cubuk2020randaugment}. Since some primitives are non-differentiable, these methods resort to reinforcement learning to learn the optimal sequence of primitives to apply. %Bayesian data augmentation \cite{tran-2017-applying} is another distinct stream of approaches which also try to learn the augmentation.

% Lastly, \textsc{DA} need not be entirely blackbox w.r.t the task model. \cite{dreossi2018counterexample} dynamically create augmented examples amidst training the task model which are close to currently misclassified examples. 

% \subsubsection{Based On Knowledge Resources}
% Lexical knowledge bases such as Wordnet \cite{miller1995wordnet} and PPDB \cite{pavlick-etal-2015-ppdb}, which annotate word-word synonymy or other, quasi-synonymous word-word relations like \emph{hypernymy}, \emph{meronymy} and \emph{paraphrase}, are a staple component of token-substitution based augmentation methods already described in \S\ref{rulebased}.

% Commonsense KBs like ATOMIC \cite{sap2019atomic} and ConceptNet \cite{speer2016conceptnet} \varun{TODO for Self} %jason i think we have enough content for section 2.2
%\begin{itemize}
%\item{Lexical Knowledge}
%\item{Commonsense Knowledge}

%\end{itemize}

%\subsubsection{Back-translation and Related Methods}
%i think this can go under "model-based techniques"
%this is a nit but we might want to avoid itemize to save sapce. idk how many model-based techinques there are, if there are a lot we might want to further subdivide
% Right I agree, don't intend to have itemize finally...was just thinking of it rn to group things, will linearize
%ok sg
%\begin{itemize}
%    \item Backtranslation %see line 20
 
%\end{itemize}

%\subsubsection{Syntactic Paraphrasing}
%i think this can go under "model-based techniques"


%\cite{yang2020g} use 
%i think this can go under "model-based techniques"
%\varun{I agree}

\subsection{How Else Might \textsc{DA} be Used?}
% \subsection{\textsc{DA} for low-resource languages} 
%\jason{I actually think this should be it's own subsection (instead of subsubsection)}
%\jason{Could start with something like: As data augmentation aims to increase the size of the training set in order to reduce overfitting, it can be especially useful for low-resource languages and scenarios where training data is rare. (Maybe cite some papers on low-resource languages and biomedical tasks)}
%\varun{Cindy}
\vspace{1.5mm} \noindent \textbf{Low-resource languages.}
One unique challenge for current NLP models is that they tend to perform poorly on languages with limited amounts of data, many of which have millions of native speakers.
\textsc{DA} has strong potential to help build competitive language-universal NLP systems that support these low-resource languages. Existing \textsc{DA} methods have both been applied on top of low-resource languages directly~\cite{fadaee-etal-2017-data,wang-etal-2018-switchout} and taken advantage of the data from related languages~\cite{xia-etal-2019-generalized}. \citet{csahin2019data} perform DA for low-resource languages by using operations on dependency trees that imitate \textit{cropping} and \textit{rotation} for image processing.

%jason: could add:
%AdvAug: Robust Adversarial Augmentation for Neural Machine Translation by Yong Cheng, Lu Jiang, Wolfgang Macherey and Jacob Eisenstein

\vspace{1.5mm} \noindent \textbf{Additional applications.}
In addition to task-agnostic augmentation, other forms of \textsc{DA} techniques have been designed with a specific application in mind. 
For example, \citet{hall-maudslay-etal-2019-name} propose counterfactual \textsc{DA}, which swaps out gendered words in a duplicated training corpus to \textbf{mitigate gender bias} in word embeddings. Innocuous label-preserving transformations (e.g. paraphrasing) have been shown to create \textbf{adversarial examples} that fool state-of-the-art NLP models \cite{jia2019certified}. Further, \citet{feng2020genaug} propose and evaluate DA methods for \textbf{text generation}, and \citet{longpre2019exploration} investigate DA techniques for \textbf{question-answering (QA)}.
% \jason{Done on my end but feel free to edit}\steven{looks good, i think this is a good brief summary. what i had written earlier was way too in-depth lol}

% \begin{itemize}
% \item \textbf{Mitigating gender bias:} There has been work exploring the mitigation of gender bias within NLP. For example, \citet{hall-maudslay-etal-2019-name} explore how augmentation can mitigate gender bias latent in word embeddings. They investigate the effectiveness of \textit{Counterfactual Data Augmentation (CDA)}, which is the duplication and augmentation of a corpus to remove bias, for example, by swapping out gendered words in the duplicated copy. They improve on CDA in two ways: randomly substituting potentially biased text to avoid replication (\textit{Counterfactual Data Substitution (CDS)}) and a name-pairing method that greatly increases the number of words that are handled (\textit{Names Intervention}). They find that the combination of CDS and Names Intervention is able to handle indirect gender bias and improve upon state-of-the-art in bias mitigation.
% \item \textbf{Text generation:} There has been some (but limited) exploration of augmentation for text generation. For example, GenAug \cite{feng2020genaug} looks at augmentation techniques for finetuning text generators such as GPT-2. They introduce and investigate a variety augmentation methods including keyword replacement and semantic text exchange [ADD CITE], and explore the effects of the amount of augmentation on the quality of the generated text. They find that keyword replacement with hypernyms and insertion of character-level synthetic noise are effective augmentation methods, and that the quality of the generated text improves up to approximately three times the amount of original data.
% \item \textbf{Adversarial:} 
% \item \textbf{Span-Based Tasks: e.g. NER, relations} 
% \end{itemize}

\vspace{1.5mm} \noindent \textbf{New directions.}
\textsc{DA} has been commonly used to improve model robustness \cite{li-etal-2017-robust,min-etal-2020-syntactic} and performance \cite{xie2019unsupervised,andreas-2020-good} on various tasks, especially when labeled training data is limited. %\varun{Robustness to what? What kind of performance?}
More recently, however, \textsc{DA} been increasingly used as a key component of self-supervised learning, particularly in vision \cite{chen2020simple}.
So far in NLP, BART \cite{lewis-etal-2020-bart} showed that predicting deleted tokens as a pre-training task can achieve similar performance as the masked language model, and \textsc{Electra} \cite{clark2020electra} found that pre-training by predicting corrupted tokens outperforms BERT given the same model size, data, and compute. 
Moving forward, we suspect that future work will continue to explore how to effectively manipulate text data for both pre-training and downstream tasks.
% \jason{Done on my end but feel free to edit}


%\subsection{What are the common techniques?}
%\paragraph{Model-agnostic} These methods generally involve rule-based~\cite{} or sampling-based~\cite{} word or phrase replacement on available annotated data.
%
%\paragraph{Model-based} These methods generally utilize a pretrained teacher model to produce pseudo data from unlabeled data.

%\subsection{Data augmentation for low-resource languages}

%\subsection{Other use cases of data augmentation}

%\subsection{Challenges and future directions}

==> sections/ethicsandimpact.tex <==
This being a survey paper, we neither collect any data nor propose or train any models.

We expect this paper to have a small positive impact with respect to the community of students at under-resourced institutions, AI system developers or research engineers working freelance or in small teams with respect to their work on domain-specific NLP datasets or projects or novel NLP tasks, especially those that have few examples on account of the expensiveness of annotation. On reading this paper, they would acquire a holistic and bird's eye view of the emerging palette of data augmentation methods, and also which ones apply to their respective tasks and resource constraints.

\steven{Question: is this "ethics and impact" section included as part of the page limit?}

==> sections/instructorinformation_tutorial.tex <==
% \steven{please add your bios and websites!}
% - The names, affiliations, and email addresses of the organizers, with one-paragraph statements of their research interests, areas of expertise, and experience in organising workshops and related events.

\noindent \textbf{Varun Gangal}, CMU LTI \\ 
\texttt{vgangal@andrew.cmu.edu} \\
\url{http://vgtomahawk.github.io/}\\
\noindent 
Varun is a PhD student at CMU LTI, advised by Eduard Hovy. His research is broadly on language generation, with specific interests in style transfer, data-to-text generation and document/story-level generation tasks. He has recently also been exploring data augmentation for generation.    \\

\noindent \textbf{Xinyi Wang}, CMU LTI \\ 
\texttt{xinyiw1@cs.cmu.edu} \\
\url{https://cindyxinyiwang.github.io/}\\
\noindent 
Xinyi is a PhD student at CMU LTI, advised by Graham Neubig. She primarily works on Machine Translation, focusing on efficient data utilization for low-resource languages, domain adaptation, and other scenarios when the data with desired properties is limited. \\

\noindent \textbf{Steven Y. Feng}, CMU LTI \\ 
\texttt{syfeng@andrew.cmu.edu} \\
\url{http://styfeng.github.io/}\\
\noindent 
Steven is an MLT student at CMU LTI, advised by Teruko Mitamura. His research interests include controllable generation and data augmentation techniques for generation tasks. \\
			
\noindent \textbf{Jason Wei}, ProtagoLabs \\ 
\texttt{jason@protagolabs.com} \\ 
\noindent 
Jason is a researcher at ProtagoLabs, a machine learning startup based in Tysons Corner, Virginia. His research topics include data augmentation, curriculum learning, and NLP for mental health. \\
		
\noindent \textbf{Soroush Vosoughi}, Dartmouth College \\ 
\texttt{soroush@dartmouth.edu} \\ 
\url{https://www.cs.dartmouth.edu/~soroush/} \\
\noindent 
Soroush Vosoughi is an assistant professor of computer science at Dartmouth College. He leads the minds, machines and society group, which is part of the machine learning lab at Dartmouth. His research interests lie at the intersection of machine learning, natural language processing, network science, and social media analytics.  \\
		
\noindent \textbf{Sarath Chandar}, Mila / Polytechnique Montreal \\ 
\texttt{sarath.chandar@mila.quebec} \\ 
\url{http://sarathchandar.in/} \\
\noindent 
Sarath Chandar is an assistant professor in the Department of Computer \& Software Engineering at École Polytechnique de Montréal. He is also a core faculty member at Mila, the Quebec AI Institute and holds a Canada CIFAR AI Chair. His research focuses on recurrent neural networks, lifelong learning, reinforcement learning and natural language processing. He has also co-organized past tutorials on Memory Augmented NNs for NLP (EMNLP'17) and Multilingual Multimodal Language Processing using NNs (NAACL'16).  \\

==> sections/readinglist_tutorial.tex <==
% \varun{About 6-7 references here, including atleast \textbf{1-2 survey papers}(We're currently missing the survey pprs (these can be book chapters or scribe notes you've liked in the past too), particularly).}
% \jason{closest thing to survey paper I could find is this: \url{https://arxiv.org/pdf/1812.04718v1.pdf}, but I only looked for 15 minutes.} \varun{Thanks! - added this one. }
% \varun{Steven: Especially once we have the general reference list}
% \steven{question: must these be professional/academic readings? i know of many sites and articles (e.g. on medium/whatever) that do a pretty good job of surveying current NLP data augmentation techniques. we could maybe add a couple of them. some examples can be found at the following google doc: \url{https://docs.google.com/document/d/1_Bv4bl_sKYG42Pk3kMMM2ao0ExBHAL_K7paVWf-lcWA/edit?usp=sharing}}
The following papers describe several popular DA methods:
\begin{itemize}[leftmargin=*,nolistsep]
    \item \citet{sennrich-etal-2016-improving}:  \textit{back-translation}, one of the most popular \textsc{DA} techniques, translates data into another language and then back to the original source language.
    \item \citet{zhang2018mixup}: the influential MixUp technique trains on convex combinations of pairs of examples and their labels.
    % \citet{chapelle2001vicinal} introduce and formalize the notion of vicinal risk minimization (VRM) as contrasted with typical empirical risk minimization (ERM). Importantly, VRM provides a theoretical skeleton to ground virtual training example based data augmentation methods, such as the influential MixUp  and its variants.
    \item \citet{wei-zou-2019-eda}: evaluation of four simple text perturbation techniques (token substitution, token insertion, token shuffling, and word dropout) on CNN and LSTM networks for text classification.
    % \item \citet{coulombe2018text} provide an extensive discussion and enumeration of easy-to-implement and practically viable data augmentation methods for text
    \item \citet{xie2019unsupervised}: an unsupervised method leverages \textsc{DA} for consistency training to achieve state-of-the-art text classification using few labeled examples.
\end{itemize}

In addition, the following blog posts and code repository could be helpful:
% \jason{steven pls add another blog post and code repo as you see fit}
% \steven{i think this is good enough for reading list}
\begin{itemize}[leftmargin=*,nolistsep]
    \item Introduction to popular text augmentation techniques: \url{https://towardsdatascience.com/data-augmentation-in-nlp-2801a34dfc28}
    \item Detailed blog post on various text DA techniques: \url{https://amitness.com/2020/05/data-augmentation-for-nlp/}
    \item Lightweight library for DA on text and audio: \url{https://github.com/makcedward/nlpaug}
    \item \texttt{python} framework for adversarial examples: \url{https://github.com/QData/TextAttack}
\end{itemize}



==> sections/tasks_backup.tex <==
In this section, we discuss several DA works for common NLP tasks.\footnoteref{note1} We focus on non-classification tasks as classification is worked on by default, and well covered in earlier sections (e.g. \S\ref{sec:techniquesandmethods} and \S\ref{sec:applications}). Numerous previously mentioned DA techniques, e.g. \cite{wei-zou-2019-eda,chen-etal-2020-finding,anaby2020not}, have been used or can be used for text classification tasks.

\subsection{Summarization}\label{tasks:3}
\citet{fabbri2020improving} investigate \textit{backtranslation} as a DA method for zero and few-shot abstractive summarization along with the use of a consistency loss inspired from ideas in UDA. \citet{parida-motlicek-2019-abstract} propose an iterative DA approach for abstractive summarization in German that uses a combination of synthetic and real summarization data, where the synthetic data is generated using the Common Crawl (German) dataset. \citet{zhu2019transforming} introduce a query-focused summarization \cite{Dang2005OverviewOD} dataset collected using Wikipedia called \textsc{WikiRef} which can be used for DA.

\subsection{Question Answering (QA)}\label{tasks:5}
\citet{longpre-etal-2019-exploration} investigate various DA and sampling techniques for domain-agnostic QA including paraphrasing by \textit{backtranslation}. \citet{yang2019data} propose a DA method using distant supervision to improve BERT finetuning for open-domain QA. \citet{riabi2020synthetic} leverage Question Generation models to produce augmented examples for zero-shot cross-lingual QA. \citet{singh2019xlda} propose \textsc{XLDA}, or \textsc{cross-lingual DA}, which substitutes a portion of the input text with its translation in another language, improving performance across multiple languages on NLI tasks including the SQuAD QA task. \citet{asai-hajishirzi-2020-logic} use logical and linguistic knowledge to generate additional training data to improve the accuracy and consistency of QA responses by models.

\begin{figure}
\begin{tabular}{@{}ll@{}}
\includegraphics[width=0.48\textwidth]{Images/LinearizationDing.png}\\
\end{tabular}
\vspace{-0.8\abovedisplayskip}
  \caption{\label{img-daga} Linearization for \emph{DAGA}, \citet{ding-etal-2020-daga}}
\vspace{-2ex}
\end{figure}

\subsection{Sequence Tagging Tasks}\label{tasks:4}
\citet{ding-etal-2020-daga} propose \textsc{DAGA}, a two-step \textsc{DA} process. First, a language model over sequences of tags and words linearized as per a certain scheme (shown in Figure \ref{img-daga}) is learned. Second, sequences are sampled from this language model and de-linearized to generate new examples. \citet{csahin2019data}, discussed in \S\ref{subsec:rule-based}, use \emph{dependency tree morphing} (Figure \ref{img-deptreemorph}) to generate additional training examples on the downstream task of part-of-speech (POS) tagging. 

\citet{dai-adel-2020-analysis} modify DA techniques proposed for sentence-level tasks for named entity recognition (NER), including \textit{label-wise token and synonym replacement}, and show improved performance using both recurrent and transformer models. \citet{zhang-etal-2020-seqmix} propose a DA method based on \textsc{MixUp} called \textsc{SeqMix} for active sequence labeling by augmenting queried samples, showing improvements on NER and Event Detection. %At each iteration, they generate extra labeled sequences, and demonstrate improved performance on NER and Event Detection. 

\subsection{Parsing Tasks}\label{tasks:7}
\citet{jia-liang-2016-data} propose \textsc{data recombination} for injecting task-specific priors unto neural semantic parsers. A %high-precision
synchronous context-free grammar (SCFG) is induced from training data, and new "recombinant",  %near-interpolated
examples are sampled from it. \citet{yu2020grappa} introduce \textsc{Grappa}, a pretraining approach for table semantic parsing, and generate synthetic question-SQL pairs via an SCFG. % akin to \citet{jia-liang-2016-data}.
\citet{andreas-2020-good} uses %the linguistic principle of
\textit{compositionality} to construct synthetic examples for downstream tasks including semantic parsing. Fragments of original examples are replaced with fragments from other examples in similar contexts. See Figure \ref{tab:andreas} for an illustration. 

\citet{vania-etal-2019-systematic} investigate DA for low-resource dependency parsing including \emph{dependency tree morphing} from \citet{csahin2019data} (Figure \ref{img-deptreemorph}) and modified \textit{nonce} sentence generation from \citet{gulordava-etal-2018-colorless}, which replaces content words with other words of the same POS, morphological features, and dependency labels.% They find improvement in both monolingual and cross-lingual scenarios.

\begin{figure}%[!ht]
\centering
\begin{tabular}{@{}ll@{}}
\includegraphics[width=0.45\textwidth]{Images/andreas.png}\\
\end{tabular}
\vspace{-0.8\abovedisplayskip}
  \caption{\label{tab:andreas} \textit{Compositionality}-based \textsc{DA}, \citet{andreas-2020-good}}
\vspace{-2ex}
\end{figure} 

\subsection{Grammatical Error Correction (GEC)}\label{tasks:9}
%GEC involves automatically correcting the grammar of a piece of text.
Lack of parallel data is typically a barrier for GEC. Various works have thus looked at DA methods for GEC. %, which can be broken down into roughly two major categories: work that makes use of additional resources, and work that adds synthetic errors to noise the text.
We discuss some here, and more can be found in Table \ref{table:additional_DA_works_GEC} in Appendix \ref{section:appendix_additional_DA_works}. 

There is work that makes use of additional resources. \citet{boyd-2018-using} use German edits from Wikipedia revision history and use those relating to GEC as augmented training data.  %\citet{mizumoto-etal-2011-mining} extract Japanese GEC training data from the revision log of a language learning SNS.
\citet{zhang2019sequencetosequence} explore multi-task transfer, or the use of annotated data from other tasks.

There is also work that adds synthetic errors to noise the text. %\citet{zhang2019sequencetosequence} explore backtranslation and feature discrimination.
\citet{wang2020controllable} investigate two approaches: token-level perturbations %(similar to \citet{wei-zou-2019-eda})
and training error generation models with a filtering strategy to keep generations with sufficient errors. \citet{grundkiewicz-etal-2019-neural} use \textit{confusion sets} generated by a spellchecker for noising. \citet{choe-etal-2019-neural} learn error patterns from small annotated samples along with \textit{POS-specific noising}.%respectively, which are two of the top scoring systems in the Restricted and Low Resource tracks of the Building Educational Applications (BEA) 2019 shared task \cite{bryant-etal-2019-bea}.

There have also been approaches to improve diversity of generated errors. \citet{wan-etal-2020-improving} investigate noising through editing the latent representations of grammatical sentences, and \citet{xie-etal-2018-noising} use a neural sequence transduction model and beam search noising procedures.

\subsection{Neural Machine Translation (NMT)}\label{tasks:10}
There are many works which have investigated DA for NMT. We highlighted some in \S\ref{sec:techniquesandmethods} and \S\ref{applications:1}, e.g. \cite{sennrich-etal-2016-improving,fadaee-etal-2017-data,xia-etal-2019-generalized}. %Many already mentioned DA approaches (e.g. in \S\ref{sec:techniquesandmethods} and \S\ref{applications:1}) can be applied for NMT.
We discuss some further ones here, and more can be found in Table \ref{table:additional_DA_works_MT} in Appendix \ref{section:appendix_additional_DA_works}.

\citet{wang-etal-2018-switchout} propose \textsc{SwitchOut}, a DA method that randomly replaces words in both source and target sentences with other random words from their corresponding vocabularies. \citet{gao-etal-2019-soft} introduce \textsc{Soft Contextual DA} that softly augments randomly chosen words in a sentence using a contextual mixture of multiple related words over the vocabulary. \citet{nguyen2020data} propose \textsc{Data Diversification} which merges original training data with the predictions of several forward and backward models.

%\citet{radhakrishnan2020colloql} investigate DA methods for translating utterances into SQL queries by augmenting the WikiSQL dataset with synthetic search-style questions. \citet{xu2018synthesizing} and \citet{xu2019modeling} propose the use of GANs for tabular data generation, particularly Tabular GAN (TGAN) and Conditional Tabular GAN (CTGAN), respectively.
\subsection{Data-to-Text NLG}\label{tasks:8}
\textit{Data-to-text NLG} refers to tasks which require generating natural language descriptions of structured or semi-structured data inputs, e.g. game score tables \cite{wiseman2017challenges}. Randomly perturbing game score values without invalidating overall game outcome is one \textsc{DA} strategy explored in game summary generation \cite{hayashi2019findings}.

%Wiki tables \cite{parikh2020totto} 
%translation of data in another format into a textual natural language format, such as representing the information in a table or SQL query using a natural language description. 

Two popular recent benchmarks are E2E-NLG \cite{duvsek2018findings} and WebNLG \cite{gardent2017webnlg}. Both involve generation from structured inputs - meaning representation (MR) sequences for former and triple sequences for latter. \citet{montella2020denoising} show performance gains on WebNLG by \textsc{DA} using Wikipedia sentences as targets and parsed OpenIE triples as inputs. \citet{tandon2018tnt} propose \textsc{DA} for E2E-NLG based on permuting the input MR sequence. \citet{kedzie2019good} inject Gaussian noise into a trained decoder's hidden states and sample diverse augmented examples from it. This %self-training loop of
sample-augment-retrain loop helps performance on E2E-NLG.  

\subsection{Open-Ended \& Conditional Generation}\label{tasks:1}
There has been limited work on DA for open-ended and conditional text generation. \citet{feng2020genaug} experiment with a suite of DA methods for finetuning GPT-2 on a low-resource domain in attempts to improve the quality (e.g. \emph{fluency}, \emph{diversity}, \emph{semantic content preservation}) of generated continuations, which they call \textsc{GenAug}. They find that \textsc{WN-Hypers} (WordNet hypernym replacement of keywords) and \textsc{Synthetic Noise} (randomly perturbing non-terminal characters in words) are useful, and that the quality of the generated text improves to a peak at approximately three times the original amount of training data.

%\subsection{Classification}\label{tasks:6}
%There are many text classification tasks and works which have investigated DA for them. We looked at some in \S\ref{sec:techniquesandmethods}, e.g. \cite{chen-etal-2020-finding,anaby2020not}. %Many already mentioned DA approaches (e.g. in \S\ref{sec:techniquesandmethods}) can be applied for text classification.
%We discuss some further ones here, and more can be found in Table \ref{table:additional_DA_works_classification} in Appendix \ref{section:appendix_additional_DA_works}.

\subsection{Dialogue}\label{tasks:2}
Most DA approaches for dialogue focus on task-oriented dialogue. We outline some below, and more can be found in Table \ref{table:additional_DA_works_dialogue} in Appendix \ref{section:appendix_additional_DA_works}.

\citet{Quan2019EffectiveDA} present sentence and word-level DA approaches for end-to-end task-oriented dialogue. \citet{louvan2020simple} propose \textsc{lightweight augmentation}, a set of word-span and sentence-level DA methods for low-resource slot filling and intent classification. %\citet{gritta2020conversation} introduce a graph-based representation of dialogues called Conversation Graph (ConvGraph) that can be used for DA by creating new dialogue paths. %\citet{gao2020paraphrase} propose a paraphrase augmented response generation (PARG) framework to improve dialogue generation. %by automatically constructing augmented paraphrased training examples based on dialogue state and act labels.

\citet{hou2018sequencetosequence} present a seq2seq DA framework to augment dialogue utterances for dialogue language understanding \cite{young-pomdp}, %which involves transforming an utterance into its semantic frames,
including a \textit{diversity rank} to produce diverse utterances. %They do so by leveraging each utterance's semantic alternatives in the training data, and the incorporation of a \textit{diversity rank} to produce diverse utterances. There has also been work investigating DA for task-oriented dialogue.
\citet{zhang2019taskoriented} propose %the DA method 
\textsc{MADA} to generate diverse responses using the property that several valid responses exist for a dialogue context. %For dialogue state tracking (DST), \citet{yin2019dialog} propose an RL-based DA approach, and \citet{song2020data} propose a simple DA algorithm to improve copy-mechanism model training.% for DST.

There is also DA work for spoken dialogue. \citet{hou-etal-2018-sequence}, \citet{kim-etal-2019-data}, \citet{zhao2019data}, and \citet{yoo2018data} investigate DA methods for dialogue and \emph{spoken language understanding} (SLU), including generative latent variable models.%[Min et al.] propose a DA method using generative latent variable models to improve the performance of spoken language understanding (SLU) models.

\subsection{Multimodal Tasks}\label{tasks:11}
DA techniques have also been proposed for multimodal tasks where aligned data for multiple modalities is required. We look at ones that involve language or text. Some are discussed below, and more can be found in Table \ref{table:additional_DA_works_multimodal} in Appendix \ref{section:appendix_additional_DA_works}.

Beginning with speech, \citet{wang2020data} propose a DA method to improve the robustness of downstream dialogue models to speech recognition errors. \citet{unknown} and \citet{renduchintala2018multimodal} propose DA methods for end-to-end \emph{automatic speech recognition} (ASR). 

Looking at images or video, \citet{9206007} learn a cross-modality matching network to produce synthetic image-text pairs for multimodal classifiers. %specifically for multimodal sentiment and emotion analysis.
\citet{atlihabert} explore DA methods such as synonym replacement and contextualized word embeddings augmentation using BERT for \emph{image captioning}. \citet{kafle2017data}, \citet{yokota-nakayama-2018-augmenting}, and \citet{tang2020semantic} propose methods for \emph{visual QA} including question generation and adversarial examples. %\cite{kafle2017data} a question generation based \textsc{DA} approach which outperforms a template approach based on the original dataset's annotation process. [Yokota and Nakayama] propose a DA framework for VQA that generates additional examples from unannotated pairs of images and captions. [Tang et al.] use generated adversarial examples for images and questions as augmented VQA training examples.
